Interactive Evolutionary Multi-Objective Optimization via Learning-to-Rank

In practical multi-criterion decision-making, it is cumbersome if a decision maker (DM) is asked to choose among a set of trade-off alternatives covering the whole Pareto-optimal front. This is a paradox in conventional evolutionary multi-objective optimization (EMO) that always aim to achieve a well balance between convergence and diversity. In essence, the ultimate goal of multi-objective optimization is to help a decision maker (DM) identify solution(s) of interest (SOI) achieving satisfactory trade-offs among multiple conflicting criteria. Bearing this in mind, this paper develops a framework for designing preference-based EMO algorithms to find SOI in an interactive manner. Its core idea is to involve human in the loop of EMO. After every several iterations, the DM is invited to elicit her feedback with regard to a couple of incumbent candidates. By collecting such information, her preference is progressively learned by a learning-to-rank neural network and then applied to guide the baseline EMO algorithm. Note that this framework is so general that any existing EMO algorithm can be applied in a plug-in manner. Experiments on $48$ benchmark test problems with up to 10 objectives fully demonstrate the effectiveness of our proposed algorithms for finding SOI.

==> makefile <==
FILE=main

all:	
	latex $(FILE)
	bibtex $(FILE)
	latex $(FILE)
	latex $(FILE)
	dvips -o $(FILE).ps $(FILE).dvi
	ps2pdf $(FILE).ps
	open $(FILE).pdf

clean:
	rm -f *.aux *.blg *.log *.bbl *.out *.bak *.synctex.gz *.synctex.gz\(busy\) *.tex~

cleanall: clean
	rm -f *.dvi $(FILE).ps $(FILE).pdf

